Differential Privacy Meets Neural Network Pruning

A major challenge in applying differential privacy to training deep neural network models is scalability.The widely-used training algorithm, differentially private stochastic gradient descent (DP-SGD), struggles with training moderately-sized neural network models for a value of epsilon corresponding to a high level of privacy protection. In this paper, we explore the idea of dimensionality reduction inspired by neural network pruning to improve the scalability of DP-SGD. We study the interplay between neural network pruning and differential privacy, through the two modes of parameter updates. We call the first mode, parameter freezing, where we pre-prune the network and only update the remaining parameters using DP-SGD. We call the second mode, parameter selection, where we select which parameters to update at each step of training and update only those selected using DP-SGD. In these modes, we use public data for freezing or selecting parameters to avoid privacy loss incurring in these steps. Naturally, the closeness between the private and public data plays an important role in the success of this paradigm. Our experimental results demonstrate how decreasing the parameter space improves differentially private training. Moreover, by studying two popular forms of pruning which do not rely on gradients and do not incur an additional privacy loss, we show that random selection performs on par with magnitude-based selection when it comes to DP-SGD training.

==> alg.tex <==
\begin{algorithm}[tb]
\caption{Example algorithm}
\label{alg:algorithm}
\textbf{Input}: Your algorithm's input\\
\textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: Your algorithm's output
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$.
\WHILE{condition}
\STATE Do some action.
\IF {conditional}
\STATE Perform task A.
\ELSE
\STATE Perform task B.
\ENDIF
\ENDWHILE
\STATE \textbf{return} solution
\end{algorithmic}
\end{algorithm}

==> alg1b.tex <==


\begin{figure}

\begin{algorithm}[H]
\caption{DP-SSGD}\label{algo:dp_grad_drop_var1}
\begin{algorithmic}[1]
\REQUIRE Tensor  $\nabla$ that contains the  gradients evaluated on each data sample in a mini-batch $S$, pruning rate $C$ (a constant) that determines the compression rate of the resulting average gradient matrix (average across data samples), norm clipping hyperparameters $\gamma$, criterium $\leftarrow \{max, rand\}$. 
\ENSURE Sparse and differentially private average gradient matrix\\
\STATE
\Function{Select-indices}{$C$, criterium, weights}  
    $I \leftarrow$ indices of weights 
    \IF{Random}
     \STATE $I_{ns}$ $\leftarrow p \cdot len(I)$ indices of $I$, selected uniformly at random 
    \ELSIF{Max}
     \STATE $I_{as} \leftarrow$ argsort(weights)
     \STATE $I_{ns} \leftarrow$ bottom $p \cdot len(I)$ indices of $I_{as}$ 
    \ENDIF
\STATE $I_s \leftarrow I \setminus I_{ns}$
\RETURN {$I_{ns}$}
\EndFunction
\STATE
\Function{DP-SGD}{$\nabla$, $I_{ns}$, $\gamma$, $\sigma$}
    \STATE We compute the average gradient matrix: $\vg = \frac{1}{B} \sum_{b=1}^S \nabla[:,s]$, where $b \in \mathcal{B}$.
    % }
    %\STATE Using the noisy $\widetilde{\vh}$, we pick an index set  for remaining output dimensions $i$'s, 
    % \sout{s.t. $\widetilde{\|\vg[i,:]\|_2^2} \geq C $. }
% \mj{
%such that $\tilde{\vh}[i] \geq C$
% }
   \STATE  We ensure  $  \nabla^2[I_s] \leq \gamma$ by clipping the squared norm by $\gamma$.
    \STATE We privatize the gradients in the selected index set,  $\nabla \leftarrow \nabla[I_s] + \vn$, where $\vn \sim \Nrm(0, \sigma^2 C^2 I)$.
    
\RETURN {$I_{ns}, I_s$}
\EndFunction
\STATE
%\STATE We iterate the following function until convergence.
\Function{DP-Sparse-SGD}{$\nabla,C, \sigma, \gamma, $ criterium, $\mathcal{B}$, weights}
    % \State $\nabla += $ residuals
    % \State Select a threshold such that $ R \%$ of $|\nabla|$ is smaller than the threshold.
    % \vspace{0.2cm}
    %\STATE Dropped $\leftarrow 0$
    % \STATE Clip each element of the gradient tensor  to be
    % less than $\gamma$, i.e., for all $i,j,s$, $|\nabla[i,j,s]| \leq \gamma$.
 
 
    
    \IF{freezing}
     \STATE $I_{ns} \leftarrow$ \Call{Select-indices}{}
    \ENDIF

    \FOR{batch $\mathcal{B}$}        
    \IF{selection}
     \STATE $I_{ns} \leftarrow$ \Call{Select-indices}{}
    \ENDIF
    \STATE $I \leftarrow \nabla[I_{ns}] = 0$
    \STATE $\nabla_{DP-SSGD} \leftarrow$ \Call{DP-SGD}{}
    \ENDFOR

    

    % is a vector of Gaussian noise.
    % \sout{\mj{compute L2 sensitivity of $\vn_g[i]$}}
    % \State residuals $\leftarrow$ $\nabla$ - Dropped
\RETURN{$\nabla_{DP-SSGD}$} 
\EndFunction
\end{algorithmic}
\end{algorithm}

 
    \caption{DP-SSGD algorithm. The algorithms consists of two parts, indices selection based on criterium and privatized gradient update. In case of freezing mode, indices selection is made only once before the training. In case of selection mode, indices are selected at every iteration. Notice we do not use any gradient information to select the indices, thus preserving privacy budget.}
    \label{fig:algo}
\end{figure}
